The passive polymer problem

In this article, we introduce a generalization of the diffusive motion of point-particles in a turbulent convective flow with given correlations to a polymer or membrane. In analogy to the passive scalar problem we call this the passive polymer or membrane problem. We shall focus on the expansion about the marginal limit of velocity-velocity correlations which are uncorrelated in time and grow with the distance x as |x|^epsilon, and epsilon small. This relation gets modified for polymers and membranes (the marginal advecting flow has correlations which are shorter ranged.) The construction is done in three steps: First, we reconsider the treatment of the passive scalar problem using the most convenient treatment via field theory and renormalization group. We explicitly show why IR-divergences and thus the system-size appear in physical observables. In a second step, we reformulate the problem in terms of a Langevin equation. This is not only interesting in its own, but also gives an efficient algorithm to determine S^{2n} numerically. In a third and final step, we generalize the Langevin treatment of a particle to polymers and membranes, or more generally to an elastic object of inner dimension D with 0 <= D <= 2. These objects can intersect each other. We also analyze what happens when self-intersections are no longer allowed.

==> appendices.tex <==
\section{Appendices}

\subsection{Some integrals}
\label{a:Some integrals}
For a $d$-dimensional rotationally invariant integral over $p$, 
which may be $\int_p=\int \rmd^d p\, \rme^{-\sum_{i=1}^d \lambda_i p_i^2}$, we have with some constant $C$
\be
\int_p =\int \rmd^d p\, \rme^{-\sum_{i=1}^d \lambda_i p_i^2}
= C \frac1{\sqrt{\prod_{i=1}^d \lambda_i}}
\ .
\ee
In the case that all $\lambda_i$ equal $\lambda$, the latter
reads with the same constant $C$ 
\be
\int \rmd^d p\, \rme^{- \lambda p^2}
= C \lambda^{-d/2} \ .
\ee
Using this, we obtain by differentiating with respect to 
$\lambda_i$ moments of $p_i$; e.g.
\bea
\left[\int_p p^2\right]^{-1}{\int_p p_1^2}&=& \frac1 d \\
\label{a:2}
\left[{\int_p (p^2)^2}\right]^{-1}{\int_p (p_1)^4}&=& \frac3 {d(d+2)} \\
\label{a:3}
\left[{\int_p (p^2)^2}\right]^{-1}{\int_p p_1^2p_2^2}&=& \frac1 {d(d+2)}
\ .
\eea
Another intelligent way of doing this is to study
\be
\int_p \rme^{- p^2/2} \rme^{ \lambda  p} = C' \rme^{-\lambda^2/2}
\ .
\ee
This yields e.g.
\be
\left[\int_p (p^2)^2\right]^{-1} \int_p (ap)(bp)(cp)(dp)
=\frac1{d(d+2)}\left[ (ab)(cd)+(ac)(bd)+(ad)(bc)\right] \ ,
\ee
where the global prefactor is most easily checked by setting 
$a=b=c=d$ and comparing with \Eq{a:2}. We need
\be
\left[ \int_p (p^2)^2\right]^{-1} \int_p (xp) (yp) (lp)^2
=\frac{1}{d(d+2)}\left( (xy) l^2 +2 (lx)(ly)\right)
\ .
\ee






==> conclusion.tex <==
\section{Conclusions}
In this article, we have shown how the multiscaling
found in   the passive scalar problem carries over to extended 
elastic objects as polymers and membranes. This was possible by 
first reformulating the problem in terms of the advection of 
particles, which then allowed for a generalization to polymers
and polymerized membranes. 
Similar to the passive
scalar case, we have calculated the anomalous exponents to first 
order in a perturbative expansion. We have also discussed, how
these quantities can be measured numerically, by studying 
the drift of two monomers, which sit on different polymers or membranes.
% We have also commented on the implications for drag reduction. 

 


==> langevin.tex <==
\section{Langevin-description of the passive scalar}
\subsection{Model and basic properties}
Let us now turn to a Langevin-description of the
passive scalar problem. 
We start from \Eq{s:FPE}
\be \label{s:FPE copy}
\left[ \p_t +v(x,t) \nabla \right] \Theta(x,t) =\nu_0 \Delta \Theta(x,t)+f(x,t)
\ .
\ee
Without the source $f(x,t)$, this can 
easily be converted into a Langevin equation. The question arises, 
how the additional term $f(x,t)$ can be incorporated. We will see
below that it corresponds to the creation and annihilation of 
particles, and that it can indeed be formulated within a Langevin
description. However, this is a question of marginal 
interest, since we had seen in the last section 
that the whole renormalization  procedure can be 
performed without ever specifying the correlations of $f(x,t)$,
just knowing that they will deliver some IR-cutoff $L$. 
We therefore start our analysis by studying \Eq{s:FPE copy}
with $f(x,t)\equiv 0$. Using standard arguments \cite{Zinn},
it is transformed into a Langevin equation for the motion of 
a particle with position $r(t) \in \R^d$. Since it will 
turn out later, that to reproduce all expectation values, 
one has to introduce $N$ particles, we will already give 
the corresponding  generalization here.  
\bea
\p_t r^i_\A(t) &=& v^i(r_\A(t),t) - \zeta_\A^i(t) \nn\\
\left< \zeta^i_\A(t) \zeta^j_\B(t') \right> &=& 2 \nu_0\delta^{ij}\delta_{\A\B} \delta (t-t')\ . 
\eea
The $vv$ correlations are the same as in \Eq{s:vvcorrel}.
The dynamic action which enforces the Langevin-equation to be
satisfied reads 
\be \label{l:dynamic action with v}
J[r,\tilde r,v,\zeta] = \sum_{\A=1}^{N} \int\rmd t \, \tilde r_\A^i(t) 
\left[ \partial_t r^i_\A(t) -v^i(r_\A(t),t) +\zeta_\A^i(t) \right]
\ .
\ee 
Averaging $\rme^{-J[r,\tilde r,v,\zeta]}$ over $\zeta$ and $v$ leads to 
\bea
J[r, \tilde r] &=& 
 \int\rmd t \,  \sum_{\A=1}^{N} \left[ \tilde r_\A^i(t) 
 \partial_t r^i_\A(t) - \nu_0\tilde r_\A^i(t)^2 \right]
 \nn\\
&&- \int \rmd t\, \frac{\rD_0}{2} \sum_{\A,\B=1}^{N}\tilde r_\A^i(t) 
\left[ \int\!
\frac{\rmd^d k}{(2\pi)^d}\, P^{ij}(k) \,\frac{\rme^{ik[r_\A(t)-r_\B(t)]}}{(k^2+m^2)^{\frac{d+\E}2}}\right]
\tilde r_\B^j(t)
\ .
\label{l:dynamic action}
\eea
Symbolically, this is written as
\be
J[r, \tilde r] = \int \rmd t  \left ( \sum_{\alpha=1}^N \left[
\DynE_{\!\A}  -\nu_0 \DynF_{\!\A} \right]
-\frac{\rD_0}{2}\sum_{\alpha,\B=1}^N {}_{\A\!}\LA_\B \right)
\ .
\ee
Free response and correlation functions are
\bea
R(\omega) = \frac 1{i\omega}  &\ ,&\quad R(t) =\Theta(t)\nn \\
C(\omega) = \frac {2\nu_0}{\omega^2}  &\ ,&\quad C(t) :=\frac1{2d}
\left< \left[ r(t)-r(0)\right]^2\right>_0 = \nu_0|t| 
\ .
\eea



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Renormalization of the dynamic action}
\label{l:Renormalization of the dynamic action}
In subsection \ref{s:Perturbative corrections...} we have
seen that in the {\em dynamic action} \eq{s:dynamic action} 
only $\nu_0$ demands a renormalization. How does this renormalization
show up in the formulation as a Langevin equation?
To answer this question, write down the first order term in $\rD_0$
from the expansion of $\rme^{-J}$:
\be \label{l:pert.term}
\frac {\rD_0}2  \sum_{\A,\B=1}^{N} \reducedbildheightrule{\LB}{0.75}_\A\!\LB
\reducedbildheightrule{\LB}{0.75}_\B
\ee
with
\bea \label{l:diagram}
\reducedbildheightrule{\LB}{0.75}_\A\!\LB
\reducedbildheightrule{\LB}{0.75}_\B
&=& \tilde r_\A^i(t) 
\left[ \int\!
\frac{\rmd^d k}{(2\pi)^d}\, P^{ij}(k) \,\frac{\rme^{ik[r_\A(t)-r_\B(t)]}}{(k^2+m^2)^{\frac{d+\E}2}}\right]
\tilde r_\B^j(t)
\ .
\eea
We now have to analyze short-distance divergences, i.e.\ what happens
if the two points come close together. This is most easily done
using the techniques of multilocal operator product expansion, 
introduced in \cite{DDG3,DDG4}, further developed in 
\cite{WieseDavid1997,Wiese1997a,Wiese1997b,WieseLedoussal1998} 
and reviewed in \cite{WieseHabil}.
By the dashed line which encircles the two fat points, we 
indicate points which come close together. We now want to 
express  ${\rme^{ik[r_\A(t)-r_\B(t)]}}$ through its normal-ordered
version $\bn{\rme^{ik[r_\A(t)-r_\B(t)]}}\en$, which does not contain
any self-contractions. This is 
\be \label{l:normal order}
{\rme^{ik[r_\A(t)-r_\B(t')]}} \, = \ \bn{\rme^{ik[r_\A(t)-r_\B(t')]}}\en
\rme^{-k^2 \frac1{2d} \EXP{[r_\A(t)-r_\B(t')]^2}{0}}
\ .
\ee
This leads to a drastic simplification: Since 
$\frac1{2d} \EXP{[r_\A(t)-r_\B(t)]^2}{0}$ equals infinity except for $\A=\B$
for which it vanishes, \Eq{l:diagram} gives 
\bea
\reducedbildheightrule{\LB}{0.75}_\A\!\LB
\reducedbildheightrule{\LB}{0.75}_\B
&=& \delta_{\A\B}\,\tilde r_\A^i(t)  \tilde r_\A^j(t) 
\left[ \int\!
\frac{\rmd^d k}{(2\pi)^d}\, P^{ij}(k) \,\frac1
{(k^2+m^2)^{\frac{d+\E}2}}\right] \nn\\
&=& \delta_{\A\B}\,\tilde r_\A(t)^2  
\left( 1-  \frac{1}{d}\right) C_d \frac{m^\E}{\E} \ ,
\eea
where $C_d$ is defined in \Eq{s:Cd def}. 
Symbolically, the diagram is written as
\be\label{l:main diag}
\DIAGind{\LB}{\DynF}m= \left( 1-  \frac{1}{d}\right) C_d \frac{m^\E}{\E} 
\ ,
\ee
which reminds of Feynman's bra and ket notation. We have added an index
$m$ to indicate the IR-cutoff.
\Eq{l:main diag} leads to the same 
renormalization for $\nu$ as given in \Eq{s:Znu} for the Focker-Planck
formulation of the problem. 

Even though equivalent, the treatment in terms of the Langevin equation
reveals one important property: The only renormalization of the dynamic
action comes from the divergence in a {\em single particle} trajectory. 
We will see later, that the renormalization of $S^n$ is due to 
multi-particle diagrams. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Simple expectation values and translation table}
In this section, we make more explicit the relation between 
the two formulations of the problem. 
What we want to calculate are expectation values of $\Theta(x,t)$.
We first observe that in the limit of $N\to \infty$
\bea \label{l:equiv1}
\Theta(x,t) ~&\longleftrightarrow&~ 
\Theta_\ind L(x,t):=
\frac1N\sum_{\A=1}^N\delta^d(r_\A(t)-x)\ .
\eea
If we do not know where the particles started, then obviously
\be
\EXP{\Theta_\ind L(x,t)}{0} = 0 \ .
\ee
This is also true for higher moments
\be \label{l:higher}
\EXP{\Theta_\ind L(x,t)^n}{0} = 0 \ .
\ee
It is important to note that the limit of $N\to \infty$ is necessary 
in order to suppress correlations coming from the same particle, 
which  in the expectation value \eq{l:higher} are of 
order $1/N$. 



Equivalently in momentum representation, when 
defining the Fourier-transform as 
\be
f(x) =\int \frac{\rmd^dk }{(2\pi)^d} f(k) \rme^{ikx}
\ee
\Eq{l:equiv1} will read:
\bea
\Theta(k,t) ~&\longleftrightarrow&~ \Theta_\ind L(k,t)
 =\frac1N\sum_{\A=1}^N\rme^{-ik r_\A(t)}\ .
\eea
We now check that the free response-function \eq{s:R mixed} of the 
Focker-Planck formulation is correctly 
reproduced. In contrast to the Focker-Planck formulation, here we 
have  to solve the initial time problem explicitly, i.e.\ suppose
that the particles start at position $x_0$ at time $t_0$.
\bea
R_\ind L(x-x_0,t-t_0) &:=& \AT{\EXP{ \Theta_\ind L(x,t)}0}{r_\A(t_0)=x_0} \Theta(t-t_0)\nn\\
&=&
\int\frac{\rmd^d k}{(2\pi)^d}
\AT{\EXP{\frac1N\sum_{\A=1}^N\rme^{ik [r_\A(t)-x]} }{0}}
{r_\A(t_0)=x_0} \Theta(t-t_0)\nn\\
&=&
\int\frac{\rmd^d k}{(2\pi)^d}
\AT{\EXP{ \frac1N\sum_{\A=1}^N\rme^{ik [r_\A(t)-r_\A(t_0)]} }{0}}
{r_\A(t_0)=x_0} \rme^{ik [x_0-x]}\Theta(t-t_0)\nn\\
&=&
\int\frac{\rmd^d k}{(2\pi)^d}
\,\rme^{-k^2 \nu_0(t-t_0)}
 \rme^{ik [x_0-x]}\Theta(t-t_0)\nn\\
&\equiv& R_\ind{FP}(x-x_0,t-t_0)
\ , \label{l:L=FP}
\eea
as given in  \Eq{s:R(x,t)}. Note that this response-function 
is a single-particle function, i.e.\ only the response
of a single particle $\A$ to a change in its (earlier) trajectory  
contributes. 

Injecting particles with a rate $f(x,t)$ at time $t$ at position $x$, 
models the corresponding term in \Eq{s:FPE}, and finally leads
to the same correlation function as in the Focker-Planck representation
\bea
C_\ind L(x,t; y,t')&=&\int\rmd t_0 \int \rmd t'_0 \int\rmd^d x_0\int\rmd^d y_0 \,
R_\ind L(x-x_0,t-t_0)R_\ind L(y-y_0,t'-t'_0) \nn\\
&&
\qquad\times\EXP{f(x_0,t_0)f(y_0,t_0')}{} \nn\\
&=& 
\int\rmd t_0 \int \rmd^d x_0\int\rmd^d y_0 \,
R_\ind L(x-x_0,t-t_0)R_\ind L(y-y_0,t'-t_0) G_f(M x_0 ,M y_0) \nn\\
&\equiv& C_\ind{FP} (x,t; y,t')\ .
\eea

By comparing the terms of order $v(x,t)$ in \Eqs{s:dynamic action with v}
 and \eq{l:dynamic action with v}, 
we also obtain the equivalence
\bea
\label{l:equiv2}
\Theta(x,t) \nabla^i\tilde \Theta(x,t) ~&\longleftrightarrow&~ 
\Theta_\ind L(x,t) \nabla^i\tilde \Theta_\ind L(x,t):=
\sum_{\A=1}^N
\tilde r_\A^i(t) \delta^d(r_\A(t)-x) \ .
\eea

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{The scaling of $S^{2n}$ and
renormalization of composite operators}
\label{l:The scaling of S(2n)...}
We now have to reproduce the results of section \ref{s:scaling of S 2n}.
This will be done in two steps. First, we will show that
the OPE of ${\cal O}^i_\ind{L}(x,t):=\Theta_\ind L(x,t)\nabla^i \tilde
\Theta_\ind L(x,t) = \sum_{\A=1}^N \tilde r^i_\A(t) \delta^d(r_\A(t)-x)$
with the $n$-th power of $\Theta_\ind L(y,t')=\frac1N \sum_{\B=1}^N 
\delta^d(r_\B(t')-y)$ is as in the formulation via a Focker-Planck
equation encoded in the contraction of ${\cal O}^i_\ind{L}(x,t)$ with a single
$\Theta_\ind L(y,t')$:
\be
{\cal O}^i_\ind{L}(x,t) \contract \Theta_\ind L(y,t')^n = n \,
\Theta_\ind L(y,t')^{n-1}\,\left[ {\cal O}^i_\ind{L}(x,t) \contract \Theta_\ind L(y,t') \right]\ .
\ee
The reason is that when contracting $\tilde r^i_\A(t)$ in ${\cal O}^i_\ind{L}(x,t)$
with $\Theta_\ind L(y,t')^n$ 
singles out a particle $\A$ in one of the $\Theta_\ind L(y,t')$. 
Correlations of this particle $\A$ with $r_\beta(t')$ in 
another of the factors $\Theta_\ind L(y,t')$
only exist for $\alpha=\B$ which is suppressed by a factor of $1/N$. 

Therefore, it is sufficient to show that 
${\cal O}^i(x,t) \contract \Theta(y,t')$
is the same in both the Focker-Planck and the Langevin
formulations. In the Focker-Planck formulation, we 
have 
\be \label{l:FP form ui}
{\cal O}^i_\ind{FP}(x,t) \contract \Theta_\ind{FP}(y,t')
=\Theta_\ind{FP}(x,t) \nabla^i R_\ind{FP}(x-y,t-t')
\ .
\ee
In the Langevin-formulation, the same expression reads
\bea
{\cal O}^i_\ind{L}(x,t) \contract \Theta_\ind{L}(y,t')
&=& \sum_{\A=1}^N \tilde r^i_\alpha(t) \delta^d(r_\A(t)-x)
\contract \frac1N \sum_{\B=1}^N \delta^d(r_\B(t')-y)
\nn\\
&=& \Theta(t'-t) 
\frac1N \sum_{\A=1}^N \int\!\frac{\rmd^d k}{(2\pi)^d}
\,\int\!\frac{\rmd^d p}{(2\pi)^d}\,(ip)^i\, \rme^{ik[r_\A(t)-x]}
\contract  \rme^{ip[r_\A(t')-y]} \nn\\
&=& \Theta(t'-t) 
\frac1N \sum_{\A=1}^N \int\!\frac{\rmd^d k}{(2\pi)^d}
\,\int\!\frac{\rmd^d p}{(2\pi)^d}\,(ip)^i\, \bn \rme^{ik[r_\A(t)-x]}
 \rme^{ip[r_\A(t')-y]}\en \rme^{kp|t-t'|} \ ,\nn\\
\eea
where the normal-order sign ``$:$'' indicates that contractions between
the included operators are factored out as $\rme^{kp|t-t'|}$.
This is useful since the normal-ordered operator $\bn \rme^{ik[r_\A(t)-x]}
\rme^{ip[r_\A(t')-y]}\en$ is free of divergences when approaching 
$x$ and $y$. For an introduction and review of these techniques, 
see \cite{WieseHabil}.


In the next step, the integration variable $k$ is shifted
to $k\to k-p$
\be
\Theta(t'-t) 
\frac1N \sum_{\A=1}^N \int\!\frac{\rmd^d k}{(2\pi)^d}
\,\int\!\frac{\rmd^d p}{(2\pi)^d}\,(ip)^i\, \bn \rme^{ik[r_\A(t)-x]}
 \rme^{ip[r_\A(t')-r_\A(t)]}\en \rme^{(k-p)p|t-t'|} \rme^{ip[x-y]}
\ .
\ee
Partially undoing the normal-order procedure finally leads to 
\be\label{l:partially undo}
\Theta(t'-t) 
\frac1N \sum_{\A=1}^N \int\!\frac{\rmd^d k}{(2\pi)^d}
\,\int\!\frac{\rmd^d p}{(2\pi)^d}\,(ip)^i\, \bn \rme^{ik[r_\A(t)-x]}
 \en\;\bn\rme^{ip[r_\A(t')-r_\A(t)]}\en \rme^{-p^2|t-t'|} \rme^{ip[x-y]}
\ .
\ee
Note that this is not the standard procedure 
(as described in \cite{WieseHabil}) but is particularly useful for 
our purposes. Two  routes of argument are now open: The first one 
consists in the observation that in the desired limit of $t\to t'$, 
$\bn\rme^{ip[r_\A(t')-r_\A(t)]}\en$ is approximately 1, and thus 
the integrals over $k$ and $p$ factorize, leading to
\be 
\Theta_\ind L(x,t)
\,\nabla^i\,R_\ind{L}(x-y,t-t') \ ,
\ee 
which using \Eq{l:L=FP} is  the same result as in \Eq{l:FP form ui}.

\begin{figure}[t]
\centerline{\epsfxsize=0.5\textwidth\epsfbox{./pictures/diffdiag.eps}}
\caption{The two different types of diagrams, involved in the renormalization
of {\em (a)} $\nu$ (left) and {\em (b)} $S^{2n}$ (right). In both cases
we have drawn the particle trajectories, as well as one interaction.}
\end{figure}%
We finally want to argue that  the above result becomes
exact, when specifying the boundary conditions. To
that purpose, suppose that we start at time $\tau$ at position 0. 
The condition that the particle be at
position 0 is again expressed as a $\delta$-function and using the Fourier-%
representation $\delta^d(r_\A(\tau))=\int\!\frac{\rmd^d l}{(2\pi)^d}\,
\rme^{ilr_\A(\tau)}$, we are led to study the expectation value of 
\be
\EXP{\rme^{ilr_\A(\tau)} \int\!\frac{\rmd^d k}{(2\pi)^d}\, \rme^{ik[r_\A(t)-x]}}0
=\int\!\frac{\rmd^d k}{(2\pi)^d} \,\rme^{kl|t-\tau|} \rme^{-ikx}
\EXP{\rme^{ilr_\A(\tau)+ikr_\A(t)}}0
\ .
\ee
Since $\EXP{\rme^{ilr_\A(\tau)+ikr_\A(t)}}0= (2\pi)^d\delta^d(k+p)$,
only expectation values of exponentials 
$$
\bn\rme^{i\sum_{j=1}^n k_j r_\A(t_j)}\en
$$
survive for which global ``charge neutrality'' $\sum_{j=1}^n k_j=0$ holds.
Therefore, in \Eq{l:partially undo}, we have to  supply an additional 
factor $\rme^{-ikr_\A(\tau)}$ at initial
time $\tau$, leading inside the integral to  
\be
\bn\rme^{ik[r_\A(t)-r_\A(\tau)]}\en \;\bn\rme^{ip[r_\A(t')-r_\A(t)]}\en \rme^{-p^2|t-t'|-k^2|t-\tau|} \ .
\ee
(Note that we have already normal-ordered the first exponential,
leading to the factor of $\rme^{-k^2|t-\tau|}$.)
The key-observation now is that
\be
\bn\rme^{ik[r_\A(t)-r_\A(\tau)]}\en \;\bn\rme^{ip[r_\A(t')-r_\A(t)]}\en
\;\equiv\; \bn\rme^{ik[r_\A(t)-r_\A(\tau)]}\rme^{ip[r_\A(t')-r_\A(t)]}\en
\ ,
\ee
as long as $\tau<t$ and (by assumption) $\tau<t'$. This factorization 
property is one of the essential simplifications for polymers (which are
nothing but a random walk), see e.g.\ section 10 of \cite{WieseHabil}.
For our case, it shows that the above stated {\em approximate}
equivalence between the Focker-Planck and Langevin descriptions is 
indeed exact, as one expects from the equivalence of the two equations. 

In conclusion: Since the above arguments show (at least at leading order)
the equivalence of the 
both perturbation theories 
for the renormalization of $S^{2n}$, we 
obtain the same results as in subsection  \ref{s:scaling of S 2n}.

Let us still give some remarks on the class of diagrams involved
in the renormalization of  $S^{2n}$. Whereas the diagrams which 
contribute to the renormalization of $\nu$ are single-particle
diagrams, i.e.\ diagrams where one particle interacts with 
itself, the diagrams which contribute to the renormalization of 
$S^{2n}(x-y)$ are multiple-particle diagrams, i.e.\ diagrams where 
one particle which finally ends at $x$ interacts with another 
particle, which finally ends at $y$. 

\subsection{Interpretation in terms of particle trajectories only}
\label{L:Interprete particle}
\begin{figure}
\centerline{\epsfxsize=0.5\textwidth\epsfbox{./pictures/particles.eps}}
\caption{Intuitive interpretation of $S^{2n}(x-y)$ via particles being
advected by the turbulent flow. Drawn is one configuration 
which contributes to  $t_{xy}$ of \protect\Eq{l:txy}.
Note that particles may return into the box, such that one has to 
wait long enough until the probability of return tends to 0.
For details cmp.\ the main text.}
\label{l:particles picture}
\end{figure}%
First of all, one can determine the single particle motion, which is 
super-diffusive.
By means of a complete RG-analysis, or faster using 
the method of exact exponent identities \cite{WieseHabil}, we obtain
due to  the non-renormalization of the terms proportional to 
$\tilde r \p_t r$ and $D_0$ the exact identity
\be
\label{l:correl exact}
\EXP{\left( r_\A(t)-r_\A(0)\right)^2}{} \sim |t|^{\frac{2}{2-\E}} \ ,
\ee
which is the analogue of \Eq{s:gamma star} ff.

More interestingly, $S^{2n}(x-y,t)$ can also be obtained in terms of 
particle trajectories only, following 
\cite{FrischMazzinoNoullezVergassola1999,FrischMazzinoVergassola1998}.
We first note that due to  \Eq{l:equiv1}, 
$\Theta_\ind L(x,t)$ is the contribution from particles which are 
created by $f(x', t')$
at time $ t'<t $ and position $x'$ and arrive
 at time $t$ at position $x$:
\be 
\Theta_\ind L(x,t) = \frac1N\sum_{\alpha=1}^N \int^t_{-\infty} \rmd 
t' \,\AT{f(r_\alpha(t'),t')}{r_\A(t)=x} \ .
\ee
This gives a simple method to evaluate  moments of $\Theta$
within a Monte Carlo simulation. The following observation
helps to render the derivation more transparent: 

 For given $\zeta$ and $v$, the process is deterministic. Since $\zeta$ and
 $v$ are 
Gaussian and uncorrelated in time,
 they are time-reversal invariant. We therefore write 
$\Theta_\ind L(x,t)$ as integral over all trajectories, starting at
time $t$ at $x$ and ending at time $t'>t$ at $x'$, where they 
are ``created'' by $f( x',t')$:
\be \label{l:Theta L}
\Theta_\ind L(x,t) = \frac1N \sum_{\alpha=1}^N \int_t^{\infty} \rmd 
t' \,{f(r^x_\A(t'),t')} \ ,
\ee
where $r_\A^x(t)$ satisfies the equation of motion 
and boundary condition
\be
\p_{t'} r_\A^x(t') = v(r_\A^x(t'),t') +\zeta_\A(t) \ , \qquad r_\A^x(t)=x \ .
\ee
We now turn to the evaluation of higher correlation functions. 
Let us demonstrate the principle on the example of the second 
moment, keeping in mind that finally $N\to \infty$:
\bea
\lefteqn{\EXP{\left[\Theta (x,t) - \Theta(y,t)\right]^2}{} =
\EXP{\EXP{
\EXP{\left[\Theta_\ind L(x,t) - \Theta_\ind L(y,t)\right]^2}{\zeta}}{f}
}{v} }\nn\\
&=&
\frac1{N^2}\!\sum_{\A,\B=1}^N \EXP{\EXP{ \EXP{\int_t^{\infty}\!\! \rmd t_1 \int_t^{\infty} \!\!\rmd t_2
\Big[f(r_\A^x(t_1),t_1){-}f(r_\A^y(t_1),t_1)\Big]
\Big[f(r_\B^x(t_2),t_2){-}f(r_\B^y(t_2),t_2)\Big]
}{\zeta}}{f}}{v} \nn\\
&=& \frac1{N^2}\!\sum_{\A,\B=1}^N \int_t^{\infty} \rmd t' 
\EXP{\EXP{ G_f^M( r_\A^x(t'),r_\B^x(t')) +G_f^M( r_\A^y(t'),r_\B^y(t') )
- 2 G_f^M( r_\A^x(t'),r_\B^y(t') )}{\zeta} }{v}  \ , \nn\\
\label{l:example for particle corr}
\eea
where we used that 
\be
\left< f(r,t) f(r',t') \right> = \delta(t-t')\, G_f(Mr,Mr')
\equiv \delta(t-t')\, G_f^M(r,r')
\ee
is $\delta$-correlated in time.
In principle, $G_f(x,y)$ has to fulfill four conditions

\begin{itemize}
\item[({\em i})] $ G_f(x,y)=G_f(y,x) $ .

\item[({\em ii})] $ \int_x G_f(x,y)=0$ as a consequence of 
$\int_r f(r,t)=0$ in order to have no global heating 
(particle conservation). This condition is necessary to reach a 
steady state.

\item[({\em iii})] $ G_f(x,y) \stackrel{x\to \infty}\llllongrightarrow 0$\ .
We take it at least exponentially decaying at scale 1.

\item[({\em iv})]  $G_f$ has to be realizable as a stochastic process, such
that as a consequence of \\ 
$\left< \left(f(x,t)-f(y,t)\right)^2\right> \ge0$ one must have    
$G_f(x,x)+G_f(y,y)-2G_(x,y) \ge 0$\ .
\end{itemize}

\noindent
A possible choice for $G_f(x,y)$ that satisfies the above conditions is
\be
G_f(x,y):= \Delta_x \Delta_y  \rme^{-x^2-y^2} = 4\, \rme^{-x^2-y^2}(2x^2-d)(2y^2-d) \ .
\ee
Constraint ({\em iv})  is satisfied since
\be
G_f(x,x)+G_f(y,y)-2\,G_f(x,y)= {4\,{\rme^{-2\left({x^2}+{y^2}\right)}}{{\left[d\left({\rme^{{x^2}}}-{e^{{y^2}}}\right)+2\,{\rme^{{y^2}}}{x^2}-2\,{\rme^{{x^2}}}{y^2}\right]}^2}} \ge 0 \ .
\ee

In simulations, people \cite{FrischMazzinoNoullezVergassola1999,%
FrischMazzinoVergassola1998}
use $G_f(x,y) = {\bf \Theta}(|x-y|<1) $ (with
$\bf \Theta$ being the step function), which violates 
condition ({\em ii}), but appearantly leads to good results.
(Particle conservation seems to be no problem, when working at  fixed
particle number. 
For another argument see \cite{FrischMazzinoNoullezVergassola1999}.) 
As explained in section \ref{s:Model}, we make the ansatz that
$G_f(x,y)$ depends both on $x$ and $y$ and not only on the difference $x-y$.
Similar in spirit to \cite{FrischMazzinoNoullezVergassola1999,%
FrischMazzinoVergassola1998}
would thus be $G_f(x,y) = {\bf \Theta}(|x|<1){\bf \Theta}(|y|<1)$.  
\Eq{l:example for particle corr} then acquires the  
form
\bea \label{l:interp2}
\lefteqn{\EXP{\left[\Theta (x,t) - \Theta(y,t)\right]^2}{} } \nn\\
&=& \frac1{N^2}\!\sum_{\A,\B=1}^N 
 \int_t^{\infty}\!\!\rmd t'\,
\EXP{\EXP{\Big[{\bf \Theta} (|r_\A^x(t')|{<}L) {-} {\bf \Theta} (|r_\A^y(t')|{<}L)\Big]
\Big[{\bf \Theta} (|r_\B^x(t')|{<}L) {-} {\bf \Theta} (|r_\B^y(t')|{<}L)\Big] }{\zeta}}{v}\ .\nn\\
\eea
We see that this is the $v$-average of a quantity which can be
interpreted as a time. 
Let us in general define 
\be \label{l:txy}
 t_{xy} := \frac1{N^2}\!\sum_{\A,\B=1}^N \int_t^{\infty} \rmd t' 
\EXP{ G_f^M( r_\A^x(t'),r_\B^x(t')) +G_f^M( r_\A^y(t'),r_\B^y(t') )
- 2 G_f^M( r_\A^x(t'),r_\B^y(t') )}{\zeta} \ .  
\ee
Then $\EXP{\left[\Theta (x,t) - \Theta(y,t)\right]^2}{}$ is
the $v$-average of $t_{xy}$:
\be \label{l:interp2p}
\EXP{\left[\Theta (x,t) - \Theta(y,t)\right]^2}{} = \EXP{ t_{xy}}{v}\ .
\ee
Analogously, for the fourth moment we can write 
using that $f$ is  Gaussian and $N\to \infty$
\bea \label{l:interp3}
\lefteqn{\hspace*{-3cm}\EXP{\left[\Theta (x,t) - \Theta(y,t)\right]^4}{} = 
\frac3{N^4}\!\sum_{\A,\B,\G,\D=1}^N \int_t^{\infty} \rmd t' \,
\int_t^{\infty}\rmd t''}\nn\\\hspace{3cm}
\bigg<\Big< &\Big[& G_f^M( r_\A^x(t'),r_\B^x(t')) +G_f^M( r_\A^y(t'),r_\B^y(t') )
- 2 G_f^M( r_\A^x(t'),r_\B^y(t') ) \Big]\times \nn\\
&\Big[&G_f^M( r_\G^x(t''),r_\D^x(t'')) +G_f^M( r_\G^y(t''),r_\D^y(t'') )
- 2 G_f^M( r_\G^x(t''),r_\D^y(t'') )\Big]\, \Big>_{\!\!\zeta}\bigg>_{\!\!v}
\nn\\
&&= 3 \EXP{\BRA{ t_{xy} }2 }{v}
\ .
\eea
In general, the $2n$-th moment is 
\be \label{l:interp2n}
\EXP{\left[\Theta (x,t) - \Theta(y,t)\right]^{2n}}{} = 
\frac{(2n)!}{2^n n!}  \EXP{\BRA{ t_{xy}}{n} }{v}
\ .
\ee
One can now easily check
the deviation from Gaussian behaviour by analyzing connected
expectation values. 
\Eq{l:interp2n} also tells us that the anomalous behaviour 
of $S^{2n}$ comes from rare large events, i.e.\ rare large
$t_{xy}$. Moreover, the measured ensemble of
$t_{xy}$
not only contains the information about the moments, but even the 
complete probability distribution function. 

Let us give some comments on simulations
\cite{FrischMazzinoVergassola1998,FrischMazzinoNoullezVergassola1999}: In the above formulation,
we have always averaged over $N$ replicas for the particles 
and their corresponding thermal noises, finally taking $N\to \infty$. 
For the $2n$-th moment, it
is indeed sufficient to keep $2n$ different particles. Moreover, 
the thermal noise can be dropped for particles which are not
starting at the same point. Finally, by going to the relative 
coordinate system, and using $G_f$ of the 
form $G_f(x-y)$, only the $2n-1$ relative coordinates have to be propagated. 

Also note that
with a little bit of work, using \Eq{l:correl exact} and the anomalous 
dimension of $(\nabla \Theta)^{2n}$, one can again obtain the anomalous 
scaling behaviour as given in \Eq{s:explicit}.


==> membrane.tex <==
\section{Generalization to polymers and membranes}
\subsection{Construction of the generalized model}
We are now in a position to generalize the above considerations
to polymers and polymerized (tethered) membranes. 

To this aim, we introduce a polymer or polymerized 
tethered membrane 
\cite{KantorKardarNelson1986a,KantorKardarNelson1986b} 
with coordinates 
\be
\gx \in \R^D ~\longrightarrow~ r(\gx) \in \R^d\ , 
\ee 
where we think of $D$ between 0 and 2, and in particular of
$D=0$ for a particle, $D=1$ for a polymer and $D=2$ for a membrane. 
For polymers, $\gx$ measures the length along the polymer; 
for membranes, $\gx$ belongs to a 2-dimensional coordinate system. 
$r(\gx)$ is the position of the monomer $\gx$ in imbedding space. 
The standard model for polymers is due to Edwards \cite{Edwards1965} 
and reads generalized to membranes \cite{KantorKardarNelson1986a,KantorKardarNelson1986b}
\be \label{m:SA membrane}
{\cal H} [r] = \int \rmd^D \gx\, \half (\nabla r(\gx))^2 
+b \int \rmd^D \gx\int \rmd^D \gy \, \delta^d(r(\gx)-r(\gy))
\ .
\ee 
The second term punishes self-intersections of the membrane, 
making the membrane self-avoiding. 
In what follows, we shall study phantom membranes, i.e.\ drop the 
term proportional to $b$. {We shall
discuss the general case in section \ref{m:Self-avoidance}.}

As for particles, we introduce $N$ 
copies, labeled by lower Greek indices. 
For the $\alpha$-th polymer, 
the equation of motion for the monomer $\gx$ at time $t$ and 
with coordinates $r_\A(\gx,t)$ then reads
\be \label{m:eqn motion}
\p_t r^i_\A(\gx,t) = \Delta_\gx r_\A^i(\gx,t) + v^i(r_\A(\gx,t),t) + \zeta_\A^i(\gx,t) 
\ .
\ee 
Note that the elasticity of the polymer or membrane has been 
scaled to 1.  
The $vv$-correlations are the same as in \Eq{s:vvcorrel},
and we already note that $\E=0$ is {\em not} the marginal case.
The thermal noise is Gaussian with zero mean and 
correlations
\bea
\left< \zeta^i_\A(\gx,t) \zeta^j_\B(\gy,t') \right> &=& 2 \nu_0\delta^{ij}\delta_{\A\B} \delta (t-t') 
\delta^D(\gx-\gy)\ .
\eea 
The dynamic action which enforces the Langevin-equation to be
satisfied reads in analogy to \Eq{l:dynamic action with v}
\be \label{m:dynamic action with v}
J[r,\tilde r,v,\zeta] = \sum_{\A=1}^{N} \int\rmd t \, 
\rmd^D\gx\,
\tilde r_\A^i(\gx,t) 
\left[ \partial_t r^i_\A(\gx,t)-\Delta_\gx r_\A^i(\gx,t) -v^i(r_\A(\gx,t),t) -\zeta_\A^i(\gx,t) \right]
\ .
\ee 
Averaging $\rme^{-J[r,\tilde r,v,\zeta]}$ over $\zeta$ and $v$ leads to 
\bea
J[r, \tilde r] &=& 
 \int\rmd t \,\rmd^D\gx \,  \sum_{\A=1}^{N} \left[ \tilde r_\A^i(\gx,t) 
 \partial_t r^i_\A(\gx,t) - \tilde r_\A^i(\gx,t) \Delta_\gx r_\A^i(\gx,t)
 - \nu_0\tilde r_\A^i(\gx,t)^2 \right]
 \nn\\
&&-\frac{\rD_0}2 \int \rmd t\,\rmd^D\gx\, \rmd^D\gy\,
 \sum_{\A,\B=1}^{N}\tilde r_\A^i(\gx,t) 
\left[ \int\!
\frac{\rmd^d k}{(2\pi)^d}\, P^{ij}(k) \,\frac{\rme^{ik[r_\A(\gx,t)-r_\B(\gy,t)]}}{(k^2+m^2)^{\frac{d+\E}2}}\right]
\tilde r_\B^j(\gy,t)
\ .\qquad
\label{m:dynamic action}
\eea 
Symbolically, this is written as
\be
J[r, \tilde r] = \int\! \rmd t\, \rmd^D\gx\, \left ( \sum_{\alpha=1}^N \left[
\DynE_{\!\A}+\DynA_{\!\A}  -\nu_0 \DynF_{\!\A} \right]\right)
-\frac{\rD_0}{2}
\int\! \rmd t\, \rmd^D\gx\, \rmd^D\gy\,
\sum_{\alpha,\B=1}^N {}_{\A\!}\LA_\B 
\ ,
\ee 
where we used the abbreviations
\bea
&&\DynE_{\!\A}= \tilde r_\A(\gx,t) \p_t r_\A(\gx,t) \ ,\qquad
\DynA_{\!\A}= \tilde r_\A(\gx,t) (-\Delta_\gx) r_\A(\gx,t) \ ,\qquad
\DynF_{\!\A}= \tilde r_\A(\gx,t)^2  \nn \\
&&{}_{\A\!}\LA_\B = \tilde r_\A^i(\gx,t) 
\left[ \int\!
\frac{\rmd^d k}{(2\pi)^d}\, P^{ij}(k) \,\frac{\rme^{ik[r_\A(\gx,t)-r_\B(\gy,t)]}}{(k^2+m^2)^{\frac{d+\E}2}}\right]
\tilde r_\B^j(\gy,t)
\ .
\eea 
The free single-membrane response- and correlation-functions are
\bea
R(\gk,\omega) = \frac 1{i\omega+\gk^2}  &\ ,&\quad R(\gk,t) =\Theta(t)
\rme^{-t \gk^2}\ ,\quad R(\gx,t)= \Theta(t) (4\pi t)^{-D/2} \rme^{-\gx^2/4t}
\nn \\
C(\gk,\omega) = \frac {2\nu_0}{\omega^2+(\gk^2)^2}  &\ ,&
\quad C(\gk,t) := \frac{\nu_0}{\gk^2}\, \rme^{-|t|\gk^2}
\ .
\eea 
At equal times,  the free correlation-function has the simple form
\be
C(\gx-\gy,0) := \frac1{2d}\EXP{\left(r(\gx,t)-r(\gy,t)\right)^2}{0}
=\frac{\nu_0}{(2-D)S_D} |\gx-\gy|^{2-D}
\ .
\ee 
All other free correlations vanish.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Renormalization of the dynamic action}
As in section \ref{l:Renormalization of the dynamic action}, 
we now have to analyze possible renormalizations of the dynamic action.
As in \Eq{l:pert.term}, we start from 
\be
\frac {\rD_0}2  \sum_{\A,\B=1}^{N} \reducedbildheightrule{\LB}{0.75}_\A\!\LB
\reducedbildheightrule{\LB}{0.75}_\B 
\ ,
\ee 
which is more explicitly
\bea \label{m:diagram}
\reducedbildheightrule{\LB}{0.75}_\A\!\LB
\reducedbildheightrule{\LB}{0.75}_\B
&=& \int\rmd^D\gy \,\tilde r_\A^i(\gx,t) 
\left[ \int\!
\frac{\rmd^d k}{(2\pi)^d}\, P^{ij}(k) \,\frac{\rme^{ik[r_\A(\gx,t)-r_\A(\gy,t)]}}{(k^2+m^2)^{\frac{d+\E}2}}\right]
\tilde r_\B^j(\gy,t)
\ .
\eea 
We will see below that contracting a response-field will give 
no contribution. We are thus left to normal-order
the r.h.s.\ of \Eq{m:diagram} by virtue of a generalization of
\Eq{l:normal order}
\be \label{m:normal order}
{\rme^{ik[r_\A(\gx,t)-r_\B(\gy,t')]}} \, = \
 \bn{\rme^{ik[r_\A(\gx,t)-r_\B(\gy,t')]}}\en
\rme^{-k^2 \frac1{2d} \EXP{[r_\A(\gx,t)-r_\B(\gy,t')]^2}{0}}
\ .
\ee
Only the term with $\A=\B$ gives a non-zero contribution: 
\be \int\rmd^D\gy \,
\tilde r_\A^i(\gx,t) 
\left[ \int\!
\frac{\rmd^d k}{(2\pi)^d}\, P^{ij}(k) \,\frac{{\bn\rme^{ik[r_\A(\gx,t)-r_\A(\gy,t)]}} \en
\rme^{-\frac{\nu_0}{(2-D)S_D}k^2|\gx-\gy|^{2-D}}}
{(k^2+m^2)^{\frac{d+\E}2}}\right]
\tilde r_\A^j(\gy,t)
\ .
\ee 
The leading UV-divergence is obtained by expanding 
$\bn {\rme^{ik[r_\A(\gx,t)-r_\A(\gy,t)]}} \en$ and keeping the term of 
order 1. (Note that such an expansion is justified since the normal-ordered
product itself does not contain any divergence.) 
Using the rotational invariance of the integration over 
$k$ yields 
\be
\tilde r_\A(\gx,t)^2  \left(1-\frac1d\right) 
\int\rmd^D\gy \,
\int \frac{\rmd^d k}{(2\pi)^d}\,
\frac{\rme^{-\frac{\nu_0}{(2-D)S_D}k^2|\gx-\gy|^{2-D}}}
{(k^2+m^2)^{\frac{d+\E}2}}
\ .
\ee 
Performing the integrals over $\gy$ and $k$ finally gives 
 the contraction of ${\LB}$ and projection onto 
$\DynF$:  
\bea 
\DIAGind{\LB}{\DynF}{m}&=&
 \left( 1-\frac1d\right)C_{d}^D\, \frac{m^{-\delta}}\delta 
 \nu_0^{-\frac D{2-D}}
 \\
 \delta &=& \E+\frac{2D}{2-D} \label{m:4.16}\\
C^D_{d}&=&
\frac{2S_D}{2-D} \left[(2-D)S_D\right]^{\frac D{2-D}}
\frac{\Gamma\left(\frac D{2-D}\right)
\Gamma\left(\frac d 2-\frac D{2-D} \right) 
\Gamma\left(1+\frac\delta2\right) }
{(4\pi)^{d/2}\Gamma\left(\frac {d+\E}{2}\right)
\Gamma\left(\frac {d}{2}\right)} \nn\\
&\!\!\stackrel{\delta\to 0}\llongrightarrow\!\!&\ \ 
\frac{2S_D}{2-D} \left[(2-D)S_D\right]^{\frac D{2-D}}
\frac{\Gamma\left(\frac D{2-D}\right)  }
{(4\pi)^{d/2}\Gamma\left(\frac {d}{2}\right)} \checked
\ .\qquad 
\eea 
This is the generalization of \Eq{l:main diag} to membranes.
We have put the index $m$ to the diagram to remind the reader
that $m$ acts as regulator. Note that now the dimensional
regularization parameter is $\delta$
instead of $\E$.

Other renormalizations for the dynamic action 
do not appear: First,  contracting in \Eq{m:diagram}
one of the response-fields, say $\tilde r_\A^i(\gx,t)$
leads to a factor of $k^i$, which together with $P^{ij}(k)$
gives 0. 
This argument is generalized to all orders in 
perturbation theory upon remarking that the same  factor 
always appears in the MOPE for the interaction which is 
 most advanced in time. One can also show that the emerging
diagrams themselves also vanish, due to a response-function 
at equal times. 

Let us now turn back to the renormalization-group functions.
Bare and renormalized couplings are
\bea
u_0&=&\frac{\rD_0}{\nu_0^{\frac2{2-D}}} = u \,\frac {Z_\ind D}{Z_\nu^{\frac2{2-D}}}\,
m^\delta \\
Z_\nu&=&1-\frac u \delta \left(1-\frac1d\right) \frac{C_d^D}2 \ ,
\qquad Z_\ind D = 1
\ .
\eea 
In analogy to \Eq{s:beta}, the $\beta$-function reads
\be
\beta(u) := m \AT{\frac \p {\p m}}{0} u = -\delta u + 
\frac{{C_d^D}}{2-D} \left(1-\frac1d\right)  u^2 + O(u^3)\checked
\ .
\ee 
It  has a non-trivial IR-attractive fixed point at
\be \label{m:u star}
u^*= \frac{(2-D)d}{C_d^D (d-1)} \,\delta\ .
\ee 
We can as in \Eq{s:gamma def} define the anomalous dimension $\gamma_{\nu}$ of 
$\nu$ as
\bea
\gamma_{\nu} (u)&:=& m \frac \p {\p m} \ln Z_\nu \nn\\
&=&u \left(1-\frac1d\right) \frac {C_d^D}2
\label{m:gamma def}
\ ,
\eea 
which at $u=u^*$ reads 
\be \label{m:gamma nu}
\gamma_{\nu}^*=\frac{2-D}{2}\D \ .
\ee 
A new exponent is associated to the equal-time inner-membrane 
correlation function
\bea
C_\ind m (\gx-\gy) &:=& \frac1{2d}\left< \left(r(\gx,t)-r(\gy,t) \right)^2\right>
\nn\\
&\sim& |\gx-\gy|^{2\kappa^*} \ .
\eea 
From \Eq{m:gamma nu} we obtain the result to 
order $\delta$
\be \label{m:kappa ord delta}
\kappa^*=\frac{2-D}2 \left(1+\frac{2-D}4\delta +O(\delta^2) \right) \ .
\ee 
Using that neither the term $\int \tilde r r$, nor $\int \tilde r (-\Delta) r$,
nor the interaction proportional to $\mathrm D_0=\mathrm D$
is renormalized, the scaling dimension of $r$ can as in \Eq{l:correl exact}
be obtained exactly:
\be \label{m:rt}
\EXP{\BRA{r_\A(\gx,t)-r_\A(\gx,t')}2}{} \sim |t-t'|^{\frac{2}{2-\E}} \ .
\ee
Since $\gx^2\sim t$
\be \label{m:kappa exact}
\EXP{\BRA{r_\A(\gx,t)-r_\A(\gy,t)}2}{} \sim |\gx-\gy|^{2\kappa^*}\ , \qquad
\kappa^*=\frac{2}{2-\E}=\frac{2}{\frac{4}{2-D}-\delta} \ .
\ee
In the limit of $\delta\to 0$, this reproduces \Eq{m:kappa ord delta}.
It is important to note that for $\E>0$, the exponent $\kappa^*$
is larger than 1, thus the membrane over-stretched, and the description
of a membrane via 
\Eq{m:SA membrane} with only a harmonic elastic
term 
${\cal H} [r] = \int \rmd^D \gx\, \half [\nabla r(\gx)]^2$
 breaks down. 
 This coincides
with the range of $\E$, for which already a single particle, hence 
the center of mass of the membrane, exhibits anomalous diffusion. 
This range will not be described by our model. 
In experiments one has indeed observed destruction of  polymers
by a turbulent flow \cite{BonnCoudervanDouady1993,CadotBonnDouady1998}.


\subsection{Higher moments: the scaling of $S^{2n}$}
\label{m:higher moments}
Let us now address the question of higher correlation functions.
 To this aim, we first have 
to generalize the particle-density $\Theta_\ind L(x,t)$ defined 
in \Eq{l:equiv1} to polymers and membranes. Be ${\cal V}:=\int \rmd^D \gx $
the volume of a membrane, then define
\be \label{m:Theta}
\Theta_\ind m(x,t) := \frac1{N{\cal V}} \sum_{\A=1}^N 
\int \rmd^D \gx\, \delta^d( r_\A(\gx,t)-x)
\ .
\ee 
Note that $\Theta_\ind m(x,t)$ has a well-defined limit both for 
$N\to\infty$ and ${\cal V} \to \infty$. Even though we average over all
monomers, it will later turn out that $\Theta_\ind m(x,t)$ can be
interpreted in terms of a single monomer, in analogy of the discussion in 
section \ref{L:Interprete particle}.

Let us again consider $S^{2n}(x,y):=\left< 
\left[\Theta_\ind m(x,t)-\Theta_\ind m(y,t) \right]^{2n}\right>$.
As in \Eq{s:2.41}, we have to study the contraction of 
$T^{ij}\nabla^i\Theta_\ind m(y,t) \nabla^j \Theta_\ind m(y,t)$ with 
$$
J_\ind{int}:\checkedequal\frac {\rD_0} 2
 \int \rmd t\,\rmd^D\gx\, \rmd^D\gx'\,
  \sum_{\A,\B=1}^{N}\tilde r_\A^a(\gx,t) 
\left[ \int\!
\frac{\rmd^d k}{(2\pi)^d}\, P^{ab}(k) \,\frac{\rme^{ik[r_\A(\gx,t)-r_\B(\gx',t)]}}{(k^2+m^2)^{\frac{d+\E}2}}\right]
\tilde r_\B^b(\gx',t)  \ .
$$
This reads
\bea
\lefteqn{T^{ij}\nabla^i\Theta_\ind m(y,t) \nabla^j \Theta_\ind m(y,t) \contract J_\ind{int}} \nn\\
&\checkedequal& -\BRA{\frac1{N{\cal V}}}{2}  \sum_{\A=1}^N \sum_{\B=1}^N
\int\!\rmd^D\gy\int\!\rmd^D\gy'
\int\!\frac{\rmd^d (p-k)}{(2\pi)^d}
\int\!\frac{\rmd^d (l+k)}{(2\pi)^d}\,
\rme^{i(p-k)[r_\A(\gy,t)-y]} \,\rme^{i(l+k)[r_\B(\gy',t)-y]}\nn\\
&& \qquad\times T^{ij}(p-k)^i (l+k)^j\nn\\
&& \contract\frac {\rD_0} 2
 \int \rmd \tau\,\rmd^D\gx\, \rmd^D\gx'\,
 \sum_{\G,\D=1}^{N}\tilde r_\G^a(\gx,t{-}\tau) 
\left[ \int\!
\frac{\rmd^d k}{(2\pi)^d}\, P^{ab}(k) \,\frac{\rme^{ik[r_\G(\gx,t{-}\tau)-r_\D(\gx',t{-}\tau)]}}{(k^2+m^2)^{\frac{d+\E}2}}\right]
\tilde r_\D^b(\gx',t{-}\tau) \ ,\nn\\
\eea 
where we have already shifted the $l$- and $p$-integration for later
convenience.
Following the partial normal ordering procedure of section 
\ref{l:The scaling of S(2n)...} and noting $\gz=\gx-\gy$, 
$\gz'=\gx'-\gy'$ leads to 
\bea
\lefteqn{T^{ij}\nabla^i\Theta_\ind m(y,t) \nabla^j \Theta_\ind m(y,t) \contract J_\ind{int}} \nn\\
&\checkedequal& \rD_0\BRA{\frac1{N{\cal V}}}{2}  \sum_{\A=1}^N \sum_{\B=1}^N
\int\!\rmd^D\gy\int\!\rmd^D\gy'
\int\!\rmd^D\gz\int\!\rmd^D\gz'
\int\!\rmd \tau
\int\!\frac{\rmd^d p}{(2\pi)^d}
\int\!\frac{\rmd^d l}{(2\pi)^d}
\int\!\frac{\rmd^d k}{(2\pi)^d} \nn\\
&&\qquad \times\, T^{ij}(p-k)^i(k+l)^j  
\frac{(p-k)^a P^{ab}(k) (k+l)^b}{(k^2+m^2)^{\frac{d+\E}2}}
\nn\\
&& \qquad \times \bn \rme^{i(p-k)[r_\A(\gy,t)-r_\A(\gx,t{-}\tau)]}\en
\rme^{ip[r_\A(\gx,t-\tau)-x]} \,\rme^{i(x-y)(p-k)-(p-k)^2 C(\gz,\tau)} R(\gz,\tau)\nn\\
&& \qquad \times \bn \rme^{i(k+l)[r_\B(\gy',t)-r_\B(\gx',t{-}\tau)]}\en
\rme^{il[r_\B(\gy,t-\tau)-x]} \,\rme^{i(x-y)(k+l)-(k+l)^2 C(\gz',\tau)} R(\gz',\tau)
\ . \qquad
\eea 
This expression allows for one exact simplification, namely
\be
{(p-k)^a P^{ab}(k)\, (k+l)^b} = {p^a P^{ab}(k)\, l^b}
\ .
\ee 
Similar to what has been done after \Eq{l:partially undo}, we use
the approximations 
\bea
\bn \rme^{i(p-k)[r_\A(\gy,t)-r_\A(\gx,t{-}\tau)]}\en &\approx&1 \nn\\
\bn \rme^{i(k+l)[r_\B(\gy',t)-r_\B(\gx',t{-}\tau)]}\en&\approx&1 \ ,
\eea 
which were exact for the particle (see the discussion in 
section \ref{l:The scaling of S(2n)...}). 

Next, since we are searching for the leading pole in $\delta=\E+\frac{2D}{2-D}$, 
which comes from the region, where $k$ becomes large and 
where $\tau, \gz$ and $\gz'$ become small simultaneously, 
we can replace $k+l$ by $k$ and $p-k$ by $-k$. This leads to
\bea
\lefteqn{T^{ij}\nabla^i\Theta_\ind m(y,t) \nabla^j \Theta_\ind m(y,t) \contract J_\ind{int}} \nn\\
&\checkedapprox& {-}\rD_0 \BRA{\frac1{N{\cal V}}}{2}  \sum_{\A=1}^N \sum_{\B=1}^N
\int \!\rmd^D\gy\,\rmd^D\gy'\,
\rmd^D\gz\,\rmd^D\gz'\,\rmd \tau\,
\frac{\rmd^d p}{(2\pi)^d}\,
\frac{\rmd^d l}{(2\pi)^d}\,
\frac{\rmd^d k}{(2\pi)^d} \, T^{ij}k^i k^j  
\frac{p^a P^{ab}(k) \,l^b}{(k^2{+}m^2)^{\frac{d+\E}2}}
\nn\\
&& \qquad \times 
\rme^{ip[r_\A(\gx,t-\tau)-x]} \,
\rme^{il[r_\B(\gy,t-\tau)-x]}\,
\rme^{-k^2 [C(\gz,\tau)+C(\gz',\tau)]} R(\gz,\tau) R(\gz',\tau)\nn\\
&\checkedequal& \rD_0
\int\!\rmd^D\gz\int\!\rmd^D\gz'\int\!\rmd\tau
\int\!\frac{\rmd^d k}{(2\pi)^d} \, T^{ij}k^i k^j  \,
\frac{ P^{ab}(k)}{(k^2+m^2)^{\frac{d+\E}2}}
\rme^{-k^2 [C(\gz,\tau)+C(\gz',\tau)]} R(\gz,\tau) R(\gz',\tau)
\nn\\
&& \qquad \times 
\nabla^a \Theta_\ind m(x,t-\tau)\,\nabla^b\Theta_\ind m(x,t-\tau)\ .
\eea 
One now has to evaluate the integral over $k$, $\gz$, $\gz'$ and $\tau$, 
with $m$ as an IR-regulator. The calculation of the leading pole in 
$\delta$ is substantially simplified by moving the regulator from 
the $k$-integration to the $\tau$-integration. For the leading pole, we
have (setting $\nu_0=1$ for calculational convenience)
\bea
\lefteqn{\rD_0\!\int\!\rmd^D\gz\int\!\rmd^D\gz'\int\!\rmd\tau\!
\int\!\frac{\rmd^d k}{(2\pi)^d} \, T^{ij}k^i k^j  \,
\frac{ P^{ab}(k)}{(k^2+m^2)^{\frac{d+\E}2}}
\rme^{-k^2 [C(\gz,\tau)+C(\gz',\tau)]} R(\gz,\tau) R(\gz',\tau)
\Theta^a_m\Theta^b_m}\nn\\
&&\checkedapprox \rD_0
\int\!\rmd^D\gz\!\int\!\rmd^D\gz'\!\int_0^{m^{\frac{-4}{2{-}D}}}\!\!\rmd\tau
\int\!\frac{\rmd^d k}{(2\pi)^d} \, T^{ij}k^i k^j  
\frac{ P^{ab}(k)}{|k|^{d+\E}}
\rme^{-k^2 [C(\gz,\tau)+C(\gz',\tau)]} R(\gz,\tau) R(\gz',\tau) 
\Theta^a_m\Theta^b_m
\ ,\!\!\nn\\
\eea 
where we have abbreviated $\Theta^a_m:=\nabla^a \Theta_\ind m(x,t-\tau)$.
Since the integral scales like $m^{-\delta}$, it can equivalently be
written as 
\bea
\lefteqn{\!\!{-}\frac {\rD_0} \delta \frac{m\p}{\p m} 
\int\!\rmd^D\gz\!\int\!\rmd^D\gz'\!\int_0^{m^\frac{-4}{2-D}}\!\!\!\!\rmd\tau\!
\int\!\frac{\rmd^d k}{(2\pi)^d} \, T^{ij}k^i k^j  
\frac{ P^{ab}(k)}{|k|^{d+\E}}
\rme^{-k^2 [C(\gz,\tau)+C(\gz',\tau)]} R(\gz,\tau)
 R(\gz',\tau)\Theta^a_m\Theta^b_m }\nn\\
&&  = \frac{4 \rD_0}{2{-}D} \frac{m^{-\delta}}\delta 
\int\!\rmd^D\gz\int\!\rmd^D\gz'
\int\!\frac{\rmd^d k}{(2\pi)^d} \, T^{ij}k^i k^j  \,
\frac{ P^{ab}(k)}{|k|^{d+\E}}
\rme^{-k^2 [C(\gz,1)+C(\gz',1)]} R(\gz,1) R(\gz',1) \Theta^a_m\Theta^b_m
\ .\!\!\nn\\
\eea 
In order to proceed, we specify $T^{ij}$ as 
\be
T^{ij} = A^2 \delta^{ij}+ B^i C^j
\ .
\ee 
The integral over $k$ can still be performed, leading to
\bea
\lefteqn{ \rD_0 \,\frac{4}{2-D}\frac{m^{-\delta}}\delta  \frac{\Gamma(1{-}\frac\E2)}{\Gamma(\frac d2)(4\pi)^{d/2}}
\int\!\rmd^D\gz\int\!\rmd^D\gz' \, 
\left[C(\gz,1)+C(\gz',1)\right]^{\frac\E2-1} R(\gz,1) R(\gz',1)}
\nn\\
&&\quad\times\left[ 
A^2(\nabla\Theta_\ind m)^2\left(1{-}\frac1d\right) 
+\frac{d{+}1}{d(d{+}2)}(BC) (\nabla\Theta_\ind m)^2 -\frac2{d(d{+}2)} (\nabla \Theta_\ind mB) (\nabla\Theta_\ind m C)
\right]
\ .\qquad \quad
\label{m:4.32}
\eea 
We now introduce the abbreviation 
\bea 
I^D :=  \frac1{C_d^D}  \frac{8}{2-D}\frac{\Gamma(1{-}\frac\E2)}{\Gamma(\frac d2)(4\pi)^{d/2}}
\int\!\rmd^D\gz\int\!\rmd^D\gz' \, 
\left[C(\gz,1)+C(\gz',1)\right]^{\frac\E2-1} R(\gz,1) R(\gz',1)\ ,\qquad
\eea 
which is understood to be evaluated at $\nu_0=1$. 
In the limit of $\delta\to0$ it reads 
\bea
I^D  &\checkedequal& \frac{4\,\Gamma\left(\frac{2}{2-D}\right)}
{S_D \left[(2-D) S_D\right]^{\frac D{2-D}}\Gamma\left( \frac{D}{2-D}\right)}
\int\!\rmd^D\gz \int\!\rmd^D\gz' \, 
\left[C(\gz,1)+C(\gz',1)\right]^{-\frac{2}{2-D}} R(\gz,1) R(\gz',1) \nn\\
&\checkedequal& \frac {4 D S_D} 
{(2-D)\left[(2-D) S_D\right]^{\frac D{2-D}}}
\int\frac{\rmd\gz}{\gz}\gz^D \int\frac{\rmd\gz'}{\gz'}(\gz')^D
\left[C(\gz,1)+C(\gz',1)\right]^{-\frac{2}{2-D}} R(\gz,1) R(\gz',1)
\ . \nn\\
\label{m:ID}
\eea 
Note that $I^D$ only depends on $D$, but not on $d$.
\begin{figure}
\AxesPictureSpecial{./pictures/ID.eps}{0.7}{D}{I^D}{0.2}{-0.26}
\caption{$I^D$ as defined in \Eq{m:ID}. The crosses have 
been obtained numerically, the solid line interpolates between theses
values.}
\label{m:ID fig}
\end{figure}
For $D\to0$, the integrals over $\gz$ and $\gz'$ get localized at
$\gz=\gz'=0$, and since in that limit $C(\gz,1)\to1$ and 
$R(\gz,1)\to1$, $I^D\to1$ and we recover our earlier results of
section \ref{s:scaling of S 2n}. For general $D$, $I^D$ is smaller 
than 1. Its explicit value is plotted in figure \ref{m:ID fig}.

With this abbreviation, \Eq{m:4.32} becomes
\be \label{m:4.35}
 \frac{\rD_0}2 \frac{m^{-\delta}}\delta  
C^D_d I^D
\left[ 
A^2 (\nabla\Theta_\ind m)^2\left(1{-}\frac1d\right) 
+\frac{d{+}1}{d(d{+}2)}(BC) (\nabla\Theta_\ind m)^2 -\frac2{d(d{+}2)} (\nabla\Theta_\ind mB) (\nabla \Theta_\ind m C)
\right]
\ .\
\ee 
Setting 
\be
{\cal S}^{(n,m)}_\ind m := z^{2n} \left[ (\nabla \Theta_\ind m)^2 \right]^{n}  (z\nabla \Theta_\ind m)^{2m}
\ee 
yields for $T^{ij}$ as in \Eq{s:Tij}
\bea
T^{ij}&=& \half \frac{\p}{\p(\nabla^i\Theta_\ind m)}\frac{\p}{\p(\nabla^j\Theta_\ind m)}
\left\{z^{2n}\left[ (\nabla \Theta_\ind m)^2 \right]^{n}  (z\nabla \Theta_\ind m)^{2m}
 \right\}\nn\\
&=&n  \delta^{ij} z^{2n}\left[ (\nabla \Theta_\ind m)^2\right]^{n-1}
(z\nabla \Theta_\ind m)^{2m} \nn\\
&&+ 2n(n-1)z^{2n}(\nabla^i\Theta_\ind m)(\nabla^j\Theta_\ind m)
\left[ (\nabla \Theta_\ind m)^2 \right]^{n-2}  (z\nabla \Theta_\ind m)^{2m}
\nn\\
&&+2nm z^{2n}\left[ z^i \nabla^j\Theta_\ind m + z^j \nabla^i\Theta_\ind m \right]
\left[ (\nabla \Theta_\ind m)^2 \right]^{n-1}  (z\nabla \Theta_\ind m)^{2m-1}
\nn\\
&&+ m (2m-1) z^{2n}
z^iz^j
\left[ (\nabla \Theta_\ind m)^2 \right]^{n}  (z\nabla \Theta_\ind m)^{2m-2}
\ .
\eea 
Insertion into \Eq{m:4.35}	gives 
\bea
\frac{\rD_0}2 \frac{m^{-\D}}\D C^D_d I^D \frac{1}{d(d+2)}
&\bigg\{& 
\left[ n(d-1)(d+2n+4m)-2m(2m-1) \right] {\cal S}^{(n,m)}_\ind m
\nn\\
&& + m (2m-1)(d+1) {\cal S}^{(n+1,m-1)}_\ind m
\bigg\}
\ .
\eea 
Reestablishing the necessary factors of $\nu_0$ gives the final result
\bea \label{m:final MOPE}
{\cal S}^{(n,m)}_\ind m \contract J_\ind{int} &\checkedequal&
{\cal S}^{(n,m)}_\ind m \frac{u}2 C^D_d I^D \frac{m^{-\delta}}\delta
\frac{1}{d(d+2)}
\left[n(d-1)(d+2n+4m)-2m(2m-1)\right] \nn\\
&+&{\cal S}^{(n+1,m-1)}_\ind m \frac{u}2 C^D_d I^D
\frac{m^{-\delta}}\delta \frac{d+1}{d(d+2)}\,
m(2m-1) \ .
\eea 
\Eq{m:final MOPE} is formally equivalent to \Eq{s:final MOPE}
upon replacing $C_d$ by $C^D_d I^D$. 
As in \Eq{s:2.55} this yields for the eigen-operators 
$\bar{\cal S}_0^{(n,m)}$
\bea
\bar{\cal S}_0^{(n,m)} &=& Z^{(n,m)} \bar{\cal S}^{(n,m)} \nn\\
Z^{(n,m)} &=& 1- \frac{u}2 \frac{C_d^D I^D}\delta \frac{1}{d(d+2)}
\left[n(d-1)(d+2n+4m)-2m(2m-1)\right] 
\eea
and with the help of 
\Eq{m:final MOPE}, we can evaluate the anomalous exponents
$\gamma^{(n,m)}$ as defined in \Eqs{s:gamma(n,m)(u)} and 
\eq{s:gamma(n,m)}:
\bea \label{m:gamma(n,m)(u)}
\gamma^{(n,m)}_\ind m(u) &:=& -m \frac\p{\p m} \ln Z^{(n,m)} \nn\\
	&=&	-\frac u 2 C_d^D  I^D \frac{1}{d(d+2)}
\left[n(d-1)(d+2n+4m)-2m(2m-1)\right]
\ .
\eea 
At the IR fixed point $u=u^*$ from \Eq{m:u star}, this reads
\be \label{m:gamma(n,m)}
\gamma^{(n,m)}_\ind m \checkedequal	-  \frac{\delta\,I^D}{(d-1)(d+2)}
\left[n(d-1)(d+2n+4m)-2m(2m-1)\right]
\ .
\ee 
The full dimension $\Delta^{(n,m)}_\ind m$ of the operator $\bar{\cal S}^{(n,m)}$  then is 
\bea \label{m:full}
\Delta^{(n,m)}_\ind m &=&  (n+m)\E  +\gamma^{(n,m)}_\ind m  \nn\\
&=& -\left(n+m \right) \frac{2D}{2-D} \nn\\
&&+
\delta \left(n+m-\frac{\delta\,I^D}{(d-1)(d+2)}
\left[n(d-1)(d+2n+4m)-2m(2m-1)\right]
 \right)\qquad
\ .
\eea
The term $(n+m)\E$ is equivalent to the corresponding term in 
\Eq{s:Delta(n,m)}. It will be derived in the next section. 
The contribution to $S^{2n}$ is due to the term for $m=0$
\be
\Delta^{(n,0)}_\ind m = n \left[ \frac{-2D}{2-D} +
\delta \left(1 - I^D\frac{d+2n}{d+2}
 \right)
\right] \ .
\ee
This gives the final result for $S^{(2n)}(r)$ with $r:=|x-y|$
\be \label{m:final}
S^{(2n)}(r) = \EXP{\left[ \Theta(x,t) - \Theta(y,t)\right]^{2n}}{}
\sim r^{n\left(\frac{4}{2-D}-\delta\right)} 
\left(\frac {r} L\right)^{n \left[ \frac{-2D}{2-D} +
\delta \left(1 -  I^D\frac{d+2n}{d+2}  \right)
\right]} 
\ .
\ee
Note that for $D>0$, $I^D<1$ and 
already the second moment ($n=1$) has an anomalous
contribution at order $\delta$
\be
\Delta^{(1,0)}_\ind m = -  \frac{2D}{2-D} +\,
\delta \left(1 -{\,I^D} 
 \right) \ .
\ee


\subsection{Physical interpretation}
In section \ref{L:Interprete particle} we have  
interpreted equal-time correlation-functions of moments of $\Theta$ as 
expectation values of moments of the time  $t_{xy}$ which is constructed
from the motion of 
particles starting at $x$ and $y$. This discussion in 
terms of particle-trajectories was quite general and can immediately 
be carried over to polymers or membranes. 
In generalisation of \Eqs{l:Theta L} and \eq{m:Theta} we write
\be \label{m:Theta m}
\Theta_\ind m(x,t) = \frac1{N\cal V}\sum_{\alpha=1}^N\int \rmd^D\gx
\int_t^{\infty} \rmd 
t' \,{f(r^x_\A(\gx,t'),t')} \ .
\ee
Again, it is to be understood that $r_\alpha^x(\gx,t')$ satisfies
the equation of motion \eq{m:eqn motion} and that $r_\alpha^x(\gx,t)=x$.
Then define $t_{xy}$ as
\bea
 t_{xy} &:=& \frac1{{\cal V}^2}\frac1{N^2}\!\sum_{\A,\B=1}^N
 \int \rmd^D \gz\, \int \rmd^D \gz'\,
  \int_t^{\infty} \rmd t'  \nn\\
&&\ \EXP{ G_f^M( r_\A^x(\gz,t'),r_\B^x(\gz',t')) +G_f^M( r_\A^y(\gz,t'),r_\B^y(\gz',t') )
- 2 G_f^M( r_\A^x(\gz,t'),r_\B^y(\gz',t') )}{\zeta} \ .  \nn\\ 
\eea
Note that the expectation value is independent of $\gz$ and 
$\gz'$ such that the average over $\gz$ and $\gz'$ can be dropped. 
 We thus can alternatively define
\bea
 t_{xy} &:=&\frac1{N^2}\!\sum_{\A,\B=1}^N  \int_t^{\infty} \rmd t'  \nn\\
&&\ \EXP{ G_f^M( r_\A^x(\gz,t'),r_\B^x(\gz',t')) +G_f^M( r_\A^y(\gz,t'),r_\B^y(\gz',t') )
- 2 G_f^M( r_\A^x(\gz,t'),r_\B^y(\gz',t') )}{\zeta} \ .  \nn\\ 
\eea
This object is the analog of \Eq{l:txy}, with a single particle $\A$
replaced by an arbitrarily chosen mononmor $\gz$ on the membrane $\A$.  

Let us now come to the evaluation of observables. 
In \Eq{m:rt}, we have seen that the scaling of time and space 
is related by $t\sim r^{2-\E}$, such that 
\be\label{m:4.54}
\left< \Theta(x,t) \Theta(y,t) \right> \sim |x-y|^{2-\E}
=|x-y|^{\frac{4}{2-D}-\delta} \ .
\ee
This result is identical to the particle case, such 
that without any proper renormalization, $(\nabla \Theta)^{2n}$
would have dimension $-n\E$, establishing the 
first term in \Eq{m:full}. \Eq{m:4.54} also yields the non $L$-dependent
term in \Eq{m:final}.

Finally, in a computer-experiment, one can then measure ($r:=|x-y|$)
\be
S^{(2n)}(r) = \EXP{\left[ \Theta(x,t) - \Theta(y,t)\right]^{2n}}{}
\sim r^{n\left(\frac{4}{2-D}-\delta\right)} 
\left(\frac {r} L\right)^{n \left[ \frac{-2D}{2-D} +
\delta \left(1 -  I^D\frac{d+2n}{d+2}  \right)
\right]} \sim \EXP{\BRA{t_{xy}}{n}}{v}
\ .
\ee
Let us state explicitly the result for polymers, which 
are probably easier to simulate than membranes. Using that the
integral $I^D$ in \Eq{m:ID} for $D=1$ gives $I^1=0.456143$, we obtain
\be
S^{(2n)}_\ind{ Polymer}(r) = \EXP{\left[ \Theta(x,t) - \Theta(y,t)\right]^{2n}}{}
\sim r^{n\left(4-\delta\right)} 
\left(\frac {r} L\right)^{n \left[ {-2} +
\delta \left(1 - 0.456143 \frac{d+2n}{d+2}  \right)
\right]} \sim \EXP{\BRA{t_{xy}}{n}}{v}
\ .
\ee
We also want to  give some practical hints:

One should best use a box of size $L$ and let particles or monomers 
start at position $\pm r/2$, with $r\ll L$, where the box extends
to $L/2$ in every direction. % Let us repeat our conclusion  of 
% section \ref{L:Interprete particle} that this is the most efficient
% way to measure $\Delta^{(n,0)}$ in a simulation. 
Also note that the evaluation of the $2n$-th moment demands to 
propagate $2n$ membranes, a number which may be reduced to 
$2n-1$ when going to the relative coordinate system.  


Another point is whether one should best measure the $L$- or the 
$r$-dependence. For particles, the best observable is the $L$-dependence,
since it directly gives the multi-scaling exponent. For polymers, 
one may instead measure what happens when $r\to \lambda r $
and $L \to \lambda^{-1} L$, since for that rescaling
\be
{S^{(2n)}_\ind{ Polymer}(r)}\ts_{r\to \lambda r\atop L \to L/\lambda}
\sim \lambda^{n\delta(1-0.912286 \frac{d+2n}{d+2})}
\ .
\ee

\subsection{Self-avoidance}\label{m:Self-avoidance}
Physical membranes are always self-avoiding, i.e.\ they are
described by model \eq{m:SA membrane} with $b>0$. One would 
therefore like to have 
 a combined treatment of self-avoidance and passive
advection. In general, such a treatment is impossible, since the
upper critical dimensions are different and not for both couplings
exists a small control parameter. In the present problem however, 
the control parameters, i.e.\ dimensions of the couplings are
\bea 
\delta := \left[u_0\right]_m = \frac{2D}{2-D}+\E  \nn\\
\gamma := \left[ b_0 \right]_\mu = 2D -\frac {2-D} 2 d
\ ,
\eea
where we have introduced a scale $\mu\sim 1/\gx$ which is common
for self-avoidance and which is related to $m$ by
\be
m = \mu^{\frac{2-D}{2}}  \ .
\ee
By choosing the range $\E$ of the turbulent advection and the 
dimension of imbedding space $d$, both $\delta$ and $\gamma$ 
can be set to zero. This is the common expansion point. 
Note that this expansion point is for $\E=-\frac d 2$, such 
that the advecting turbulent field is indeed long-range correlated. 
Short-range correlated turbulent disorder
is principally different, since under renormalization
it  generates potential disorder, and physics is 
described by a new universal fixed point. At least this
has been observed for static disorder in \cite{WieseLedoussal1998}.

Let us now turn to a diagrammatic analysis. The most complicated
diagrams come form  the correction to self-avoidance by the turbulent
advection and vice versa. First of all, the turbulent advection is
long-range correlated and thus not corrected by self-avoidance,
which is short-range. On the other hand, the turbulent advection 
can correct self-avoidance through the diagram
\be
\DIAG \LC \DynB \ ,
\ee
where we have denoted with 
\be
\DynB=2\int\rmd^D \gx \int \rmd^D \gy \int \frac{\rmd^dk}
{(2\pi)^d} \tilde r(\gx,t)  (ik) \rme^{ik[r(\gx,t)-r(\gy,t)]}
\ee
 the self-avoidance interaction. Explicitly calculating the
diagram \suppressmargin{\fbox{SA1}} shows that due to the 
transversal projector in the turbulent advection, the MOPE
coefficient
\be
\MOPE \LC \DynB
\ee
identically vanishes. 
This substantially simplifies the analysis, since now only
the correction to the fields and to the scaling of time 
intervenes in the RG-analysis. We therefore introduce renormalized
fields $r$, $\tilde r$ and a renormalized time. To this aim, 
we replace throughout this article $r\to r_0$ and $\tilde r\to \tilde r_0$, 
as well as $t \to \lambda_0 t$. 
This procedure is more formal than that employed in 
the rest of this article, but necessary to obtain the renormalization group
$\beta$-functions. 
Define (again denoting with subscript $_0$ bare quantities)
\bea
r_0 = \sqrt{Z} r \nn\\
\tilde r_0 = \sqrt{\tilde Z} \tilde r \nn\\
\lambda_0 = Z_\lambda \lambda \ .
\eea
This gives the dynamic action (with summation over the replicas
and integration variables suppressed, setting also $\nu_0\to 1$),
for which we first give the bare, and second the renormalized version: 
\bea
J[r, \tilde r] &=& \int
\DynE_0+\lambda_0 \DynA_0  -\lambda_0 \DynF_0 
-\frac{u_0\lambda_0}{2} \LA_0 + b_0 \lambda_0 \DynB_0  \nn\\
 &=& \int \!
\sqrt{Z\tilde Z}\DynE+ \sqrt{Z\tilde Z} Z_\lambda
\lambda \DynA  - Z_\lambda \tilde Z \lambda \DynF 
-\frac{u\lambda}{2} Z_u \LA + b \lambda Z_b \DynB 
\ .\nn\\
\eea
Since there is no counter-term for $\DynE$, 
\be
\tilde Z Z =1 \ .
\ee
Second, from the term proportional to $\DynA$ which is 
corrected by self-avoidance, we obtain
\be
Z_\lambda= Z_\lambda \sqrt{\tilde Z Z} = 1-\frac{b}\gamma (2-D) 
\DIAGind{\GH}{\GO}{\gamma}
\ ,
\ee
where we have used the static notation \cite{WieseDavid1997,WieseHabil}, 
since the dynamic diagrams involved in the renormalization of self-avoidance
can all be reduced to static ones \cite{Wiese1997a,WieseHabil}.
We recall the notation (see e.g.\ \cite{WieseHabil}) that 
$\DIAGind{\GH}{\GO}{\gamma}$ means the residue of the pole in 
$1/\gamma$ of the diagram $\DIAGind{\GH}{\GO}{L}$. The latter
is defined as the integral over the MOPE-coefficient
$\MOPE{\GH}{\GO}$, cut off 
at scale $L$. The diagram and $Z$-factor is as defined in 
\cite{WieseDavid1997}, where a different normalization 
was used. However the final result is only sensitive to the 
ratio of diagrams; moreover since as discussed above
there is no diagram mixing $b$ and $u$, the result only depends on 
the ratio of the two diagrams involved in the renormalization 
of pure self-avoidance. We shall therefore in the following 
treat overall normalizations  rather sloppily. 

The term proportional to $\DynF$ is only renormalized by the 
turbulent advection  \cite{Wiese1997a,WieseHabil} and reads
\be
Z_\lambda \tilde Z = 1 -\half \frac u \delta \DIAGind \LB \DynF \delta
\ .
\ee
These relations can be solved for $Z$
\be \label{m:Z}
Z= \frac 1{\tilde Z} = \frac{Z_\lambda}{\tilde Z Z_\lambda}
= 1-\frac{b}\gamma (2-D) \DIAGind{\GH}{\GO}{\gamma}
+\half \frac u \delta \DIAGind \LB \DynF \delta
\ .
\ee
The relation between bare and renormalized couplings for 
the turbulent advection are in the absence of a proper 
renormalization of $u$, i.e.\ $Z_u=1$
\bea
u_0 &=& u m^\delta \tilde Z^{-1}Z^{-\E/2} Z_\lambda^{-1}
= u m^\delta Z^{1-\E/2}Z_\lambda^{-1} \nn\\
&=& u m^\delta \left( 1-\frac{b}\gamma D \DIAGind{\GH}{\GO}{\gamma}
+\frac u \delta 
\frac{1}{2-D}\DIAGind \LB \DynF \delta
\right) \ ,
\eea
leading to the $\beta_u$-function
\be \label{m:beta u}
\beta_u(b,u):=m \AT{\frac\p{\p m}}{0} u 
= u\left[-\delta -b \frac{2D}{2-D}\DIAGind{\GH}{\GO}{\gamma}
+ u \frac{1}{2-D}\DIAGind \LB \DynF \delta \right]
\ .
\ee
Self-avoidance is renormalized by
\be
Z_b = 1+ \frac b\gamma \DIAGind{\GM}{\GB}{\gamma} \ ,
\ee
$b_0$ and $b$ are thus related by
\bea
b_0 &=& b \mu^\gamma Z_b Z_\lambda^{-1} Z^{(d+1)/2}\tilde Z^{-\half} \nn\\
&=&b \mu^\gamma \left( 1+ \frac b\gamma \DIAGind{\GM}{\GB}{\gamma}
-\frac{b}{\gamma}\frac{2-D}{2}d \DIAGind\GH\GO\gamma 
+\frac u \delta \frac{d+2}{4}\DIAGind\LB\DynF\delta
\right)
\ .\qquad\nn\\
\eea
This gives the $\beta_b$-function
\bea \label{m:beta b}
\beta_b(b,u)&:=& \mu \AT{\frac\p {\p\mu}}0 b \nn\\
\qquad&=&\!\!b\left[-\gamma \!+\! b\,  \DIAGind{\GM}{\GB}{\gamma}
\!-\!b\, {\frac{2{-}D}{2}}d \DIAGind\GH\GO\gamma 
\!+\!u\, {\frac{2{-}D}{2}\frac{d{+}2}{4}}\DIAGind\LB\DynF\delta
\right]
\ .\nn\\
\eea
\Eqs{m:beta b} and \eq{m:beta u} determine the critical point,
and \eq{m:Z} then gives the size-exponent 
\bea
\kappa(b,u) &:=& \frac{2-D}{2} -\half \mu \AT{\frac{\p}{\p\mu}}0 \ln Z \\
&=& \frac{2-D}{2}\left[1 -b \DIAGind{\GH}{\GO}{\gamma}
+\frac u 4 \DIAGind \LB \DynF \delta\right]  
\eea
at this critical point. 

\begin{figure}[t]
\centerline{\AxesPicture{./pictures/flow0.6.eps}{0.31}{b}{u}
\hspace*{-2mm}\AxesPicture{./pictures/flow1.5.eps}{0.31}{b}{u}
\hspace*{-2mm}\AxesPicture{./pictures/flow2.5.eps}{0.31}{b}{u}}
\caption{Flow of \Eqs{m:flow system} for $\delta=1$, and
$\gamma=0.6$, $\gamma=1.5$, $\gamma=2.5$ respectively.}
\end{figure}
For the remainder of this section, and to allow for a simpler analysis, 
we will specify to polymers. We also use our freedom in reparametrization 
of $u$ to set $\DIAGind \LB \DynF \delta=1$.
This gives the system of equations
\bea
\beta_u(b,u)
&=& u\left[-\delta +b + u \right] \nn\\
\beta_b(b,u) \label{m:flow system}
&=&b\left[-\gamma + 2 b
+\frac34 u\right]\\
\kappa(b,u) &=&\half \left[1+\frac b2 + \frac u 4\right] \nn
\ .
\eea
We can distinguish three fixed points:
\begin{itemize}
\item[({\em i})] The pure turbulence fixed point $u^*=\delta$ and $b^*=0$
is stable for $\gamma<\frac34\delta$. The value of $\kappa$ is
$\kappa^*=\half +\frac\delta8$. 
\item[({\em ii})] The pure self-avoidance fixed point $b^*=\frac\gamma2$
 and $u^*=0$
is stable for $\gamma>2\delta$.
 The value of $\kappa$ is
$\kappa^*=\half +\frac\gamma8$.
\item[({\em iii})] The mixed fixed point $b^*=\frac45 \gamma -\frac35 \delta$,
$u^*=\frac85 \delta -\frac45 \gamma$ is stable for $\frac34\delta<
\gamma<2\delta$. The value of $\kappa$ at the fixed point is 
$\kappa^*=\half +\frac\delta{20}+\frac\gamma{10}$.
\end{itemize}
Note that {({\em i})} and {({\em ii})} reproduce the result 
of the preceding sections and for self-avoiding polymers respectively. 
This completes the discussion of properties of a single self-avoiding
polymer (or membrane) in a turbulent flow. 

The next question is how multiple membrane properties, especially 
the scaling functions $S^{2n}$ are modified. Two routes may be 
taken: either one considers real physical membranes which are 
mutually self-avoiding. However, then already the expectation value
of $\Theta_\ind m(x,t)^2$ would vanish, since never two monomers
can arrive at the same point $x$ at time $t$, due to self-avoidance. 
Interesting expectation values are 
$\Theta_\ind m(x,t) \Theta_\ind m(y,t)$. In the case of no 
turbulent advection, they are known as contact exponets 
\cite{NelsonInJerusalemWinterSchool1989,DDG4,WieseHabil}; 
they are also related to the scaling dimension of 
operators in scalar field-theory. 

The other possible generalization, which is less physical, is to 
impose self-avoidance only between monomers of the same membrane. Then, the 
diagrams evaluated in section \ref{m:higher moments} are complete
and one simply has to use the modified expressions for $\kappa^*$
and for the fixed-point value of $u$ in order to obtain the 
new multiscaling exponents. 

It should also be possible to take into account the back-reaction
of the membrane on itself, at least approximately. A treatment
\`a la Zimm \cite{Zimm1956} would in generalization to \cite{Wiese1997b}
lead to a triple $\E$-expansion, namely in $d-4$, $D-1$ and $\delta$.

We leave the exploration of these ideas for future research. 









% \subsection{Drag reduction}
% As mentioned in the introduction, the addition of small quantities
% of polymers to a fluid drastically reduces the amount 
% of drag. What can our present calculations say about that problem:
% The most important observation is that in a fully developed
% turbulent flow, $\E=4/3$ and thus the polymer will be overstretched.
% One should therefore observe destruction of at least longer polymers
% in a real turbulent flow. This has indeed been observed 
% \cite{BonnCoudervanDouady1993,CadotBonnDouady1998}. 
% On the other hand, if the standard interpretation of 
%  the polymer as an elastic object which stores 
% energy and thus prevents it from beeing dissipated, is correct, 
% it should be most effective, when it is still elastic, thus at
% $\E$ negative. This is in agreement with the observation in 
% \cite{CadotBonnDouady1998} that only for sufficiently smooth
% forcing drag reduction is effective. 
% A more quantitative analysis of the above sketched scenario is necessary
% and is left for future research. 
% 










